On Recovering from Run-time Misbehaviour in ADR

We propose a monitoring mechanism for recording the evolution of systems after certain computations, maintaining the history in a tree-like structure. Technically, we develop the monitoring mechanism in a variant of ADR (after Architectural Design Rewriting), a rule-based formal framework for modelling the evolution of architectures of systems. The hierarchical nature of ADR allows us to take full advantage of the tree-like structure of the monitoring mechanism. We exploit this mechanism to formally define new rewriting mechanisms for ADR reconfiguration rules. Also, by monitoring the evolution we propose a way of identifying which part of a system has been affected when unexpected run-time behaviours emerge. Moreover, we propose a methodology to suggest reconfigurations that could potentially lead the system in a non-erroneous state.

==> eptcsdata.tex <==
\providecommand{\firstpage}{68}
\providecommand{\publicationstatus}{M. Carbone, I. Lanese, A. Lluch-Lafuente, A. Sokolova (Eds.):\\
6th Interaction and Concurrency Experience (ICE 2013)\\
EPTCS 131, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.131.7}{10.4204/EPTCS.131.7}}
\pdfoutput=1

